Towards Adaptive Unknown Authentication for Universal Domain Adaptation by Classifier Paradox

Universal domain adaptation (UniDA) is a general unsupervised domain adaptation setting, which addresses both domain and label shifts in adaptation. Its main challenge lies in how to identify target samples in unshared or unknown classes. Previous methods commonly strive to depict sample "confidence" along with a threshold for rejecting unknowns, and align feature distributions of shared classes across domains. However, it is still hard to pre-specify a "confidence" criterion and threshold which are adaptive to various real tasks, and a mis-prediction of unknowns further incurs misalignment of features in shared classes. In this paper, we propose a new UniDA method with adaptive Unknown Authentication by Classifier Paradox (UACP), considering that samples with paradoxical predictions are probably unknowns belonging to none of the source classes. In UACP, a composite classifier is jointly designed with two types of predictors. That is, a multi-class (MC) predictor classifies samples to one of the multiple source classes, while a binary one-vs-all (OVA) predictor further verifies the prediction by MC predictor. Samples with verification failure or paradox are identified as unknowns. Further, instead of feature alignment for shared classes, implicit domain alignment is conducted in output space such that samples across domains share the same decision boundary, though with feature discrepancy. Empirical results validate UACP under both open-set and universal UDA settings.

==> sn-sample-bib.tex <==
% \documentclass[pdflatex,sn-apa]{sn-jnl}
% \begin{document}
% 	\nocite{*}
% 	\bibliography{sn-bibliography.bib} %.bib文件名字
% \end{document}

\begin{thebibliography}{}
\providecommand{\doi}[1]{\url{https://doi.org/#1}}
\bibcommenthead

\bibitem [\protect \citeauthoryear {%
Ben-David%
\ \protect \BOthers {.}}{%
Ben-David%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2010}}%
}]{%
ben2010theory}
\APACinsertmetastar {%
ben2010theory}%
\begin{APACrefauthors}%
Ben-David, S.%
, Blitzer, J.%
, Crammer, K.%
, Kulesza, A.%
, Pereira, F.%
\BCBL {} Vaughan, J.W.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2010}{}{}.
\newblock
{\BBOQ}\APACrefatitle {A theory of learning from different domains} {A theory
  of learning from different domains}.{\BBCQ}
\newblock
\APACjournalVolNumPages{Machine learning}{79}{1}{151--175}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Bousmalis%
, Trigeorgis%
, Silberman%
, Krishnan%
\BCBL {}\ \BBA {} Erhan%
}{%
Bousmalis%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2016}}%
}]{%
bousmalis2016domain}
\APACinsertmetastar {%
bousmalis2016domain}%
\begin{APACrefauthors}%
Bousmalis, K.%
, Trigeorgis, G.%
, Silberman, N.%
, Krishnan, D.%
\BCBL {} Erhan, D.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2016}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Domain separation networks} {Domain separation
  networks}.{\BBCQ}
\newblock
\APACjournalVolNumPages{Advances in neural information processing
  systems}{29}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Bucci%
, Loghmani%
\BCBL {}\ \BBA {} Tommasi%
}{%
Bucci%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2020}}%
}]{%
bucci2020effectiveness}
\APACinsertmetastar {%
bucci2020effectiveness}%
\begin{APACrefauthors}%
Bucci, S.%
, Loghmani, M.R.%
\BCBL {} Tommasi, T.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2020}{}{}.
\newblock
{\BBOQ}\APACrefatitle {On the effectiveness of image rotation for open set
  domain adaptation} {On the effectiveness of image rotation for open set
  domain adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {European Conference on Computer Vision} {European conference
  on computer vision}\ (\BPGS\ 422--438).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Cao%
, Ma%
, Long%
\BCBL {}\ \BBA {} Wang%
}{%
Cao%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2018}}%
}]{%
cao2018partial}
\APACinsertmetastar {%
cao2018partial}%
\begin{APACrefauthors}%
Cao, Z.%
, Ma, L.%
, Long, M.%
\BCBL {} Wang, J.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2018}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Partial adversarial domain adaptation} {Partial
  adversarial domain adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the European Conference on Computer Vision
  (ECCV)} {Proceedings of the european conference on computer vision (eccv)}\
  (\BPGS\ 135--150).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Choi%
, Jeong%
, Kim%
\BCBL {}\ \BBA {} Kim%
}{%
Choi%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2019}}%
}]{%
choi2019pseudo}
\APACinsertmetastar {%
choi2019pseudo}%
\begin{APACrefauthors}%
Choi, J.%
, Jeong, M.%
, Kim, T.%
\BCBL {} Kim, C.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2019}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Pseudo-labeling curriculum for unsupervised domain
  adaptation} {Pseudo-labeling curriculum for unsupervised domain
  adaptation}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:1908.00262}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Fu%
, Cao%
, Long%
\BCBL {}\ \BBA {} Wang%
}{%
Fu%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2020}}%
}]{%
fu2020learning}
\APACinsertmetastar {%
fu2020learning}%
\begin{APACrefauthors}%
Fu, B.%
, Cao, Z.%
, Long, M.%
\BCBL {} Wang, J.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2020}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Learning to detect open classes for universal domain
  adaptation} {Learning to detect open classes for universal domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {European Conference on Computer Vision} {European conference
  on computer vision}\ (\BPGS\ 567--583).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Ganin%
\ \protect \BOthers {.}}{%
Ganin%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2016}}%
}]{%
ganin2016domain}
\APACinsertmetastar {%
ganin2016domain}%
\begin{APACrefauthors}%
Ganin, Y.%
, Ustinova, E.%
, Ajakan, H.%
, Germain, P.%
, Larochelle, H.%
, Laviolette, F.%
\BDBL {}Lempitsky, V.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2016}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Domain-adversarial training of neural networks}
  {Domain-adversarial training of neural networks}.{\BBCQ}
\newblock
\APACjournalVolNumPages{The journal of machine learning
  research}{17}{1}{2096--2030}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
He%
, Zhang%
, Ren%
\BCBL {}\ \BBA {} Sun%
}{%
He%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2016}}%
}]{%
he2016deep}
\APACinsertmetastar {%
he2016deep}%
\begin{APACrefauthors}%
He, K.%
, Zhang, X.%
, Ren, S.%
\BCBL {} Sun, J.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2016}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Deep residual learning for image recognition} {Deep
  residual learning for image recognition}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE conference on computer vision and
  pattern recognition} {Proceedings of the ieee conference on computer vision
  and pattern recognition}\ (\BPGS\ 770--778).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Hendrycks%
\ \BBA {} Gimpel%
}{%
Hendrycks%
\ \BBA {} Gimpel%
}{%
{\protect \APACyear {2016}}%
}]{%
hendrycks2016baseline}
\APACinsertmetastar {%
hendrycks2016baseline}%
\begin{APACrefauthors}%
Hendrycks, D.%
\BCBT {}\ \BBA {} Gimpel, K.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2016}{}{}.
\newblock
{\BBOQ}\APACrefatitle {A baseline for detecting misclassified and
  out-of-distribution examples in neural networks} {A baseline for detecting
  misclassified and out-of-distribution examples in neural networks}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:1610.02136}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Hinton%
, Vinyals%
, Dean%
\BCBL {}\ \protect \BOthers {.}}{%
Hinton%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2015}}%
}]{%
hinton2015distilling}
\APACinsertmetastar {%
hinton2015distilling}%
\begin{APACrefauthors}%
Hinton, G.%
, Vinyals, O.%
, Dean, J.%
\BCBL {}\ \BOthersPeriod {.}\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2015}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Distilling the knowledge in a neural network}
  {Distilling the knowledge in a neural network}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:1503.02531}{2}{7}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Krasin%
\ \protect \BOthers {.}}{%
Krasin%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2017}}%
}]{%
krasin2017openimages}
\APACinsertmetastar {%
krasin2017openimages}%
\begin{APACrefauthors}%
Krasin, I.%
, Duerig, T.%
, Alldrin, N.%
, Ferrari, V.%
, Abu-El-Haija, S.%
, Kuznetsova, A.%
\BDBL {}others%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Openimages: A public dataset for large-scale multi-label
  and multi-class image classification} {Openimages: A public dataset for
  large-scale multi-label and multi-class image classification}.{\BBCQ}
\newblock
\APACjournalVolNumPages{Dataset available from https://github.
  com/openimages}{2}{3}{18}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Li%
, Kang%
, Zhu%
, Wei%
\BCBL {}\ \BBA {} Yang%
}{%
Li%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2021}}%
}]{%
li2021domain}
\APACinsertmetastar {%
li2021domain}%
\begin{APACrefauthors}%
Li, G.%
, Kang, G.%
, Zhu, Y.%
, Wei, Y.%
\BCBL {} Yang, Y.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2021}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Domain consensus clustering for universal domain
  adaptation} {Domain consensus clustering for universal domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition} {Proceedings of the ieee/cvf conference on computer
  vision and pattern recognition}\ (\BPGS\ 9757--9766).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Liang%
, Hu%
, Feng%
\BCBL {}\ \BBA {} He%
}{%
Liang%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2021}}%
}]{%
liang2021umad}
\APACinsertmetastar {%
liang2021umad}%
\begin{APACrefauthors}%
Liang, J.%
, Hu, D.%
, Feng, J.%
\BCBL {} He, R.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2021}{}{}.
\newblock
{\BBOQ}\APACrefatitle {UMAD: Universal Model Adaptation under Domain and
  Category Shift} {Umad: Universal model adaptation under domain and category
  shift}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:2112.08553}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Liu%
, Cao%
, Long%
, Wang%
\BCBL {}\ \BBA {} Yang%
}{%
Liu%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2019}}%
}]{%
liu2019separate}
\APACinsertmetastar {%
liu2019separate}%
\begin{APACrefauthors}%
Liu, H.%
, Cao, Z.%
, Long, M.%
, Wang, J.%
\BCBL {} Yang, Q.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2019}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Separate to adapt: Open set domain adaptation via
  progressive separation} {Separate to adapt: Open set domain adaptation via
  progressive separation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition} {Proceedings of the ieee/cvf conference on computer
  vision and pattern recognition}\ (\BPGS\ 2927--2936).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Long%
, Cao%
, Wang%
\BCBL {}\ \BBA {} Jordan%
}{%
Long%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2015}}%
}]{%
long2015learning}
\APACinsertmetastar {%
long2015learning}%
\begin{APACrefauthors}%
Long, M.%
, Cao, Y.%
, Wang, J.%
\BCBL {} Jordan, M.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2015}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Learning transferable features with deep adaptation
  networks} {Learning transferable features with deep adaptation
  networks}.{\BBCQ}
\newblock
 \APACrefbtitle {International conference on machine learning} {International
  conference on machine learning}\ (\BPGS\ 97--105).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Long%
, Zhu%
, Wang%
\BCBL {}\ \BBA {} Jordan%
}{%
Long%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2017}}%
}]{%
long2017deep}
\APACinsertmetastar {%
long2017deep}%
\begin{APACrefauthors}%
Long, M.%
, Zhu, H.%
, Wang, J.%
\BCBL {} Jordan, M.I.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Deep transfer learning with joint adaptation networks}
  {Deep transfer learning with joint adaptation networks}.{\BBCQ}
\newblock
 \APACrefbtitle {International conference on machine learning} {International
  conference on machine learning}\ (\BPGS\ 2208--2217).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Padhy%
\ \protect \BOthers {.}}{%
Padhy%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2020}}%
}]{%
padhy2020revisiting}
\APACinsertmetastar {%
padhy2020revisiting}%
\begin{APACrefauthors}%
Padhy, S.%
, Nado, Z.%
, Ren, J.%
, Liu, J.%
, Snoek, J.%
\BCBL {} Lakshminarayanan, B.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2020}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Revisiting one-vs-all classifiers for predictive
  uncertainty and out-of-distribution detection in neural networks} {Revisiting
  one-vs-all classifiers for predictive uncertainty and out-of-distribution
  detection in neural networks}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:2007.05134}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Pan%
, Yao%
, Li%
, Ngo%
\BCBL {}\ \BBA {} Mei%
}{%
Pan%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2020}}%
}]{%
pan2020exploring}
\APACinsertmetastar {%
pan2020exploring}%
\begin{APACrefauthors}%
Pan, Y.%
, Yao, T.%
, Li, Y.%
, Ngo, C\BHBI W.%
\BCBL {} Mei, T.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2020}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Exploring category-agnostic clusters for open-set domain
  adaptation} {Exploring category-agnostic clusters for open-set domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition} {Proceedings of the ieee/cvf conference on computer
  vision and pattern recognition}\ (\BPGS\ 13867--13875).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Panareda~Busto%
\ \BBA {} Gall%
}{%
Panareda~Busto%
\ \BBA {} Gall%
}{%
{\protect \APACyear {2017}}%
}]{%
panareda2017open}
\APACinsertmetastar {%
panareda2017open}%
\begin{APACrefauthors}%
Panareda~Busto, P.%
\BCBT {}\ \BBA {} Gall, J.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Open set domain adaptation} {Open set domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE international conference on computer
  vision} {Proceedings of the ieee international conference on computer
  vision}\ (\BPGS\ 754--763).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Paszke%
\ \protect \BOthers {.}}{%
Paszke%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2017}}%
}]{%
paszke2017automatic}
\APACinsertmetastar {%
paszke2017automatic}%
\begin{APACrefauthors}%
Paszke, A.%
, Gross, S.%
, Chintala, S.%
, Chanan, G.%
, Yang, E.%
, DeVito, Z.%
\BDBL {}Lerer, A.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Automatic differentiation in pytorch} {Automatic
  differentiation in pytorch}.{\BBCQ}
\newblock

\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Peng%
\ \protect \BOthers {.}}{%
Peng%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2019}}%
}]{%
peng2019moment}
\APACinsertmetastar {%
peng2019moment}%
\begin{APACrefauthors}%
Peng, X.%
, Bai, Q.%
, Xia, X.%
, Huang, Z.%
, Saenko, K.%
\BCBL {} Wang, B.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2019}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Moment matching for multi-source domain adaptation}
  {Moment matching for multi-source domain adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF international conference on
  computer vision} {Proceedings of the ieee/cvf international conference on
  computer vision}\ (\BPGS\ 1406--1415).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Peng%
\ \protect \BOthers {.}}{%
Peng%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2017}}%
}]{%
peng2017visda}
\APACinsertmetastar {%
peng2017visda}%
\begin{APACrefauthors}%
Peng, X.%
, Usman, B.%
, Kaushik, N.%
, Hoffman, J.%
, Wang, D.%
\BCBL {} Saenko, K.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Visda: The visual domain adaptation challenge} {Visda:
  The visual domain adaptation challenge}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:1710.06924}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Ranjan%
, Castillo%
\BCBL {}\ \BBA {} Chellappa%
}{%
Ranjan%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2017}}%
}]{%
ranjan2017l2}
\APACinsertmetastar {%
ranjan2017l2}%
\begin{APACrefauthors}%
Ranjan, R.%
, Castillo, C.D.%
\BCBL {} Chellappa, R.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {L2-constrained softmax loss for discriminative face
  verification} {L2-constrained softmax loss for discriminative face
  verification}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:1703.09507}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Russakovsky%
\ \protect \BOthers {.}}{%
Russakovsky%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2015}}%
}]{%
russakovsky2015imagenet}
\APACinsertmetastar {%
russakovsky2015imagenet}%
\begin{APACrefauthors}%
Russakovsky, O.%
, Deng, J.%
, Su, H.%
, Krause, J.%
, Satheesh, S.%
, Ma, S.%
\BDBL {}others%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2015}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Imagenet large scale visual recognition challenge}
  {Imagenet large scale visual recognition challenge}.{\BBCQ}
\newblock
\APACjournalVolNumPages{International journal of computer
  vision}{115}{3}{211--252}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Saenko%
, Kulis%
, Fritz%
\BCBL {}\ \BBA {} Darrell%
}{%
Saenko%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2010}}%
}]{%
saenko2010adapting}
\APACinsertmetastar {%
saenko2010adapting}%
\begin{APACrefauthors}%
Saenko, K.%
, Kulis, B.%
, Fritz, M.%
\BCBL {} Darrell, T.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2010}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Adapting visual category models to new domains}
  {Adapting visual category models to new domains}.{\BBCQ}
\newblock
 \APACrefbtitle {European conference on computer vision} {European conference
  on computer vision}\ (\BPGS\ 213--226).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Sagiroglu%
\ \BBA {} Sinanc%
}{%
Sagiroglu%
\ \BBA {} Sinanc%
}{%
{\protect \APACyear {2013}}%
}]{%
sagiroglu2013big}
\APACinsertmetastar {%
sagiroglu2013big}%
\begin{APACrefauthors}%
Sagiroglu, S.%
\BCBT {}\ \BBA {} Sinanc, D.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2013}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Big data: A review} {Big data: A review}.{\BBCQ}
\newblock
 \APACrefbtitle {2013 international conference on collaboration technologies
  and systems (CTS)} {2013 international conference on collaboration
  technologies and systems (cts)}\ (\BPGS\ 42--47).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Saito%
, Kim%
, Sclaroff%
, Darrell%
\BCBL {}\ \BBA {} Saenko%
}{%
Saito%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2019}}%
}]{%
saito2019semi}
\APACinsertmetastar {%
saito2019semi}%
\begin{APACrefauthors}%
Saito, K.%
, Kim, D.%
, Sclaroff, S.%
, Darrell, T.%
\BCBL {} Saenko, K.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2019}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Semi-supervised domain adaptation via minimax entropy}
  {Semi-supervised domain adaptation via minimax entropy}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF International Conference on
  Computer Vision} {Proceedings of the ieee/cvf international conference on
  computer vision}\ (\BPGS\ 8050--8058).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Saito%
, Kim%
, Sclaroff%
\BCBL {}\ \BBA {} Saenko%
}{%
Saito%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2020}}%
}]{%
saito2020universal}
\APACinsertmetastar {%
saito2020universal}%
\begin{APACrefauthors}%
Saito, K.%
, Kim, D.%
, Sclaroff, S.%
\BCBL {} Saenko, K.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2020}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Universal domain adaptation through self supervision}
  {Universal domain adaptation through self supervision}.{\BBCQ}
\newblock
\APACjournalVolNumPages{Advances in neural information processing
  systems}{33}{}{16282--16292}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Saito%
\ \BBA {} Saenko%
}{%
Saito%
\ \BBA {} Saenko%
}{%
{\protect \APACyear {2021}}%
}]{%
saito2021ovanet}
\APACinsertmetastar {%
saito2021ovanet}%
\begin{APACrefauthors}%
Saito, K.%
\BCBT {}\ \BBA {} Saenko, K.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2021}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Ovanet: One-vs-all network for universal domain
  adaptation} {Ovanet: One-vs-all network for universal domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF International Conference on
  Computer Vision} {Proceedings of the ieee/cvf international conference on
  computer vision}\ (\BPGS\ 9000--9009).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Saito%
, Watanabe%
, Ushiku%
\BCBL {}\ \BBA {} Harada%
}{%
Saito%
, Watanabe%
\BCBL {}\ \protect \BOthers {.}}{%
{\protect \APACyear {2018}}%
}]{%
saito2018maximum}
\APACinsertmetastar {%
saito2018maximum}%
\begin{APACrefauthors}%
Saito, K.%
, Watanabe, K.%
, Ushiku, Y.%
\BCBL {} Harada, T.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2018}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Maximum classifier discrepancy for unsupervised domain
  adaptation} {Maximum classifier discrepancy for unsupervised domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE conference on computer vision and
  pattern recognition} {Proceedings of the ieee conference on computer vision
  and pattern recognition}\ (\BPGS\ 3723--3732).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Saito%
, Yamamoto%
, Ushiku%
\BCBL {}\ \BBA {} Harada%
}{%
Saito%
, Yamamoto%
\BCBL {}\ \protect \BOthers {.}}{%
{\protect \APACyear {2018}}%
}]{%
saito2018open}
\APACinsertmetastar {%
saito2018open}%
\begin{APACrefauthors}%
Saito, K.%
, Yamamoto, S.%
, Ushiku, Y.%
\BCBL {} Harada, T.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2018}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Open set domain adaptation by backpropagation} {Open set
  domain adaptation by backpropagation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the European Conference on Computer Vision
  (ECCV)} {Proceedings of the european conference on computer vision (eccv)}\
  (\BPGS\ 153--168).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Sun%
\ \BBA {} Saenko%
}{%
Sun%
\ \BBA {} Saenko%
}{%
{\protect \APACyear {2016}}%
}]{%
sun2016deep}
\APACinsertmetastar {%
sun2016deep}%
\begin{APACrefauthors}%
Sun, B.%
\BCBT {}\ \BBA {} Saenko, K.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2016}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Deep coral: Correlation alignment for deep domain
  adaptation} {Deep coral: Correlation alignment for deep domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {European conference on computer vision} {European conference
  on computer vision}\ (\BPGS\ 443--450).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Tzeng%
, Hoffman%
, Zhang%
, Saenko%
\BCBL {}\ \BBA {} Darrell%
}{%
Tzeng%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2014}}%
}]{%
tzeng2014deep}
\APACinsertmetastar {%
tzeng2014deep}%
\begin{APACrefauthors}%
Tzeng, E.%
, Hoffman, J.%
, Zhang, N.%
, Saenko, K.%
\BCBL {} Darrell, T.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2014}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Deep domain confusion: Maximizing for domain invariance}
  {Deep domain confusion: Maximizing for domain invariance}.{\BBCQ}
\newblock
\APACjournalVolNumPages{arXiv preprint arXiv:1412.3474}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Venkateswara%
, Eusebio%
, Chakraborty%
\BCBL {}\ \BBA {} Panchanathan%
}{%
Venkateswara%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2017}}%
}]{%
venkateswara2017deep}
\APACinsertmetastar {%
venkateswara2017deep}%
\begin{APACrefauthors}%
Venkateswara, H.%
, Eusebio, J.%
, Chakraborty, S.%
\BCBL {} Panchanathan, S.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2017}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Deep hashing network for unsupervised domain adaptation}
  {Deep hashing network for unsupervised domain adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE conference on computer vision and
  pattern recognition} {Proceedings of the ieee conference on computer vision
  and pattern recognition}\ (\BPGS\ 5018--5027).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
S.~Wu%
\ \protect \BOthers {.}}{%
S.~Wu%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2019}}%
}]{%
wu2019improving}
\APACinsertmetastar {%
wu2019improving}%
\begin{APACrefauthors}%
Wu, S.%
, Zhong, J.%
, Cao, W.%
, Li, R.%
, Yu, Z.%
\BCBL {} Wong, H\BHBI S.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2019}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Improving domain-specific classification by
  collaborative learning with adaptation networks} {Improving domain-specific
  classification by collaborative learning with adaptation networks}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the AAAI Conference on Artificial Intelligence}
  {Proceedings of the aaai conference on artificial intelligence}\ (\BVOL~33,
  \BPGS\ 5450--5457).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
X.~Wu%
\ \protect \BOthers {.}}{%
X.~Wu%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2021}}%
}]{%
wu2021entropy}
\APACinsertmetastar {%
wu2021entropy}%
\begin{APACrefauthors}%
Wu, X.%
, Zhang, S.%
, Zhou, Q.%
, Yang, Z.%
, Zhao, C.%
\BCBL {} Latecki, L.J.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2021}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Entropy Minimization Versus Diversity Maximization for
  Domain Adaptation} {Entropy minimization versus diversity maximization for
  domain adaptation}.{\BBCQ}
\newblock
\APACjournalVolNumPages{IEEE Transactions on Neural Networks and Learning
  Systems}{}{}{}.
\newblock

\newblock

\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Yang%
, Shi%
, Wang%
, Li%
\BCBL {}\ \BBA {} Qi%
}{%
Yang%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2021}}%
}]{%
yang2021st3d}
\APACinsertmetastar {%
yang2021st3d}%
\begin{APACrefauthors}%
Yang, J.%
, Shi, S.%
, Wang, Z.%
, Li, H.%
\BCBL {} Qi, X.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2021}{}{}.
\newblock
{\BBOQ}\APACrefatitle {St3d: Self-training for unsupervised domain adaptation
  on 3d object detection} {St3d: Self-training for unsupervised domain
  adaptation on 3d object detection}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition} {Proceedings of the ieee/cvf conference on computer
  vision and pattern recognition}\ (\BPGS\ 10368--10378).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
You%
, Long%
, Cao%
, Wang%
\BCBL {}\ \BBA {} Jordan%
}{%
You%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2019}}%
}]{%
you2019universal}
\APACinsertmetastar {%
you2019universal}%
\begin{APACrefauthors}%
You, K.%
, Long, M.%
, Cao, Z.%
, Wang, J.%
\BCBL {} Jordan, M.I.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2019}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Universal domain adaptation} {Universal domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF conference on computer vision and
  pattern recognition} {Proceedings of the ieee/cvf conference on computer
  vision and pattern recognition}\ (\BPGS\ 2720--2729).
\PrintBackRefs{\CurrentBib}

\bibitem [\protect \citeauthoryear {%
Yu%
, Hashimoto%
\BCBL {}\ \BBA {} Ushiku%
}{%
Yu%
\ \protect \BOthers {.}}{%
{\protect \APACyear {2021}}%
}]{%
yu2021divergence}
\APACinsertmetastar {%
yu2021divergence}%
\begin{APACrefauthors}%
Yu, Q.%
, Hashimoto, A.%
\BCBL {} Ushiku, Y.%
\end{APACrefauthors}%
\unskip\
\newblock
\APACrefYearMonthDay{2021}{}{}.
\newblock
{\BBOQ}\APACrefatitle {Divergence Optimization for Noisy Universal Domain
  Adaptation} {Divergence optimization for noisy universal domain
  adaptation}.{\BBCQ}
\newblock
 \APACrefbtitle {Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition} {Proceedings of the ieee/cvf conference on computer
  vision and pattern recognition}\ (\BPGS\ 2515--2524).
\PrintBackRefs{\CurrentBib}

\end{thebibliography}

